Using Video Game Development to Motivate Program Design and Algebra Among Inner-City High School Students

Introducing inner-city high school students to program design presents unique challenges. The typical assumptions of an introductory programming course, like students understand what variables and functions are, may not be safe. Therefore, asking students to define functions as part of the program design process may be an overwhelming task. Many students do not understand that a function is an abstraction over similar expressions and that parameters represent the differences among these expressions. This articles presents a novel approach to teaching program design to high school students while simultaneously reinforcing high school algebra. The approach is based on a design recipe to help students develop the abstractions that lead to functions. Using a bottom-up approach, students are taught how to abstract over similar expressions. They are then taught how to use high school algebra concepts, like compound functions and function composition, to also design functions. In addition, the article also presents empirical data collected from students to measure their reaction to the course. For the students in the course, the empirical data suggests that high school algebra concepts are successfully reinforced and that students feel they become better problem solvers, find programming intellectually stimulating, and walk away with an interest in programming.

==> eptcsdata.tex <==
\providecommand{\firstpage}{78}
\providecommand{\publicationstatus}{J. Hage (Ed.): Trends in Functional Programming\\
in Education 2019 and 2020 (TFPIE '19 and '20)\\
EPTCS 321, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.321.5}{10.4204/EPTCS.321.5}}
\pdfoutput=1

